Lagrangian Duality in 3D SLAM: Verification Techniques and Optimal Solutions

State-of-the-art techniques for simultaneous localization and mapping (SLAM) employ iterative nonlinear optimization methods to compute an estimate for robot poses. While these techniques often work well in practice, they do not provide guarantees on the quality of the estimate. This paper shows that Lagrangian duality is a powerful tool to assess the quality of a given candidate solution. Our contribution is threefold. First, we discuss a revised formulation of the SLAM inference problem. We show that this formulation is probabilistically grounded and has the advantage of leading to an optimization problem with quadratic objective. The second contribution is the derivation of the corresponding Lagrangian dual problem. The SLAM dual problem is a (convex) semidefinite program, which can be solved reliably and globally by off-the-shelf solvers. The third contribution is to discuss the relation between the original SLAM problem and its dual. We show that from the dual problem, one can evaluate the quality (i.e., the suboptimality gap) of a candidate SLAM solution, and ultimately provide a certificate of optimality. Moreover, when the duality gap is zero, one can compute a guaranteed optimal SLAM solution from the dual problem, circumventing non-convex optimization. We present extensive (real and simulated) experiments supporting our claims and discuss practical relevance and open problems.

==> SDPsolver.tex <==
%!TEX root = main.tex


\section{ADMM Solver}

\spacing

==> experiments2.tex <==
%!TEX root = main.tex


2) Verification 2 for realistic scenarios.

3) In some problem instance, state of the art fail, but we can use 
Proposition 4 to obtain a primal optimal solution, on relative small problems.

\bit
\item verification
	\bit
	\item verification1: present a bunch of test scenarios (real tests, simulations), and compare in a table
	$\candidate$ (from GN), versus $d^\star$ (with timing to compute $d^\star$). 
	Message: we can use the first verification technique to discern good from bad solutions.
	\item Manhattan world in 2D: random generation of the scenario
	\item verification1: small tests in grid world. As in Carlone15icra, we can show histograms 
	with $f^\star, d^\star$. Message: the duality gap is zero in many cases, when noise is moderate.
	Show that for increasing levels of noise $f^\star = d^\star$, but at some point it breaks 
	(this can also be due to failures to compute $f^\star$). 
	\item verification2: large problems (grid, torus, loop): test $\vxx_{GN}$
	\item verification2: standard datasets (sphereHard, rim, cubicle, others?): test $\vxx_{GN}$.
	For this last case, also show cases in which $\vxx_{GN}$ fails. 
	Message: the second way is less informative (does not compute duality/suboptimality gap) 
	but it is very efficient and its computational cost is negligible. 
	\eit
\item primal solutions (small tests in grid world)
	\bit
	\item percentage of cases with SZEP for different noise in rotation and translation?
	Message: duality gap is zero in many cases.
	\item $f^\star$ VS $f_{GN}$ (and possibly VS $f_{GN}$ with initialization).
	Message: duality can cope with cases in which the state of the art fails, while being 
	less efficient from a computational standpoint.
	\eit
\eit

%%%%%%%%%%%%%%%%
\begin{figure*}[t]
\begin{minipage}{\textwidth}%\vspace{-3mm}
% \vspace{-5mm}
% \hspace{4mm}
\begin{tabular}{cccc}%
\begin{minipage}{4cm}%
\centering%
\includegraphics[scale=0.25]{figures/gray} \\
(a)
\end{minipage}
& 
\begin{minipage}{4cm}%
\centering%
\includegraphics[scale=0.25]{figures/dualityGapBars_randomGrid3D_side3_sT10_sR20_rot} \\
(b)
\end{minipage}
& 
\begin{minipage}{4cm}%
\centering %
\includegraphics[scale=0.25]{figures/gray} \\
(c) n
\end{minipage}
& 
\begin{minipage}{4cm}%
\centering%
\includegraphics[scale=0.25]{figures/gray} \\
(d) time
\end{minipage}
\end{tabular}%
\end{minipage}%
\caption{\label{fig:local}
Verification 1 is effective: duality gap is small.
However, Verification 1 is too slow to be practical
}
\vspace{-0.5cm}
\end{figure*}


%%%%%%%%%%%%%%%%
\begin{figure}[t]
\begin{minipage}{\textwidth}%\vspace{-3mm}
% \vspace{-5mm}
% \hspace{4mm}
\begin{tabular}{cc}%
\begin{minipage}{4cm}%
\centering%
\includegraphics[scale=0.25]{figures/gray} \\
\end{minipage}
&
\begin{minipage}{4cm}%
\centering%
\includegraphics[scale=0.25]{figures/gray} \\
\end{minipage}
\end{tabular}%
\end{minipage}%
\caption{\label{fig:local}
Verification 2 can correctly discern good from bad, and is much faster
}
\vspace{-0.5cm}
\end{figure}

==> figureGrid.tex <==
%!TEX root = main.tex


\begin{figure}[t]
\centering%
\includegraphics[scale=0.3, trim=0cm 1.5cm 0cm 0cm,clip]{figures/grid} 
\vspace{-0.3cm}
\caption{\label{fig:grid} 
\grid
}
\vspace{-0.3cm} 
\end{figure}


==> figureVerification1.tex <==
%!TEX root = main.tex


%% V1
%%%%%%%%%%%%%%%%
\begin{figure*}[t]
\begin{minipage}{\textwidth}%\vspace{-3mm}
% \vspace{-5mm}
% \hspace{4mm}
\begin{tabular}{cccc}%
\begin{minipage}{4cm}%
\centering%
\includegraphics[scale=0.28]{figuresStatistics/dualityGapBars_randomGrid3D_side5_sT120_sR5_tran} \\
(a)
\end{minipage}
& 
\begin{minipage}{4cm}%
\centering%
\includegraphics[scale=0.28]{figuresStatistics/dualityGapBars_randomGrid3D_side5_sT10_sR20_rot} \\
(b)
\end{minipage}
& 
\begin{minipage}{4cm}%
\centering %
\includegraphics[scale=0.28]{figuresStatistics/dualityGapBars_randomGrid3D_side6_sT10_sR5_n} \\
(c) n
\end{minipage}
& 
\begin{minipage}{4cm}%
\centering%
\includegraphics[scale=0.28]{figuresStatistics/timeSDP_randomGrid3D_side6_sT10_sR5_n} \\
(d) time
\end{minipage}
\end{tabular}%
\end{minipage}%
\caption{\label{fig:local}
Verification 1 is effective: duality gap is small.
However, Verification 1 is too slow to be practical
}
\vspace{-0.5cm}
\end{figure*}

==> figureVerification2.tex <==
%!TEX root = main.tex


%% V2
%%%%%%%%%%%%%%%%
\begin{figure*}[t]
\begin{minipage}{\textwidth}%\vspace{-3mm}
% \vspace{-5mm}
% \hspace{4mm}
\begin{tabular}{cccc}%
\begin{minipage}{4cm}%
\centering%
\includegraphics[scale=0.28]{figuresStatistics/precisionRecall_randomGrid3D_side5_sT120_sR5_tran} \\
(a)
\end{minipage}
& 
\begin{minipage}{4cm}%
\centering%
\includegraphics[scale=0.28]{figuresStatistics/precisionRecall_randomGrid3D_side5_sT10_sR20_rot} \\
(b)
\end{minipage}
& 
\begin{minipage}{4cm}%
\centering %
\includegraphics[scale=0.28]{figuresStatistics/precisionRecall_randomGrid3D_side6_sT10_sR5_n} \\
(c) n
\end{minipage}
& 
\begin{minipage}{4cm}%
\centering%
\includegraphics[scale=0.28]{figuresStatistics/timeVerify2_randomGrid3D_side6_sT10_sR5_n} \\
(d) time
\end{minipage}
\end{tabular}%
\end{minipage}%
\caption{\label{fig:local}
Verification 1 is effective: duality gap is small.
However, Verification 1 is too slow to be practical
}
\vspace{-0.5cm}
\end{figure*}

==> maps.tex <==
%!TEX root = main.tex

\definecolor{dgreen}{rgb}{0,0.5,0}
\vspace{-0.1cm}

% \newcommand{\textwidth}{9cm}
\newcommand{\widthCol}{3cm}

\begin{figure}[t]
\begin{minipage}{8.5cm}%\vspace{-3mm}
% \hspace{4mm}
\begin{tabular}{ccc}%
& {\sphereHard} & \hspace{1cm} {\torus} 
\vspace{-0.1cm}
\\
%%%%%%% FIRST ROW
\begin{sideways}{$\!\!\!\!\!\!\!\!\!\!\!$\color{green}{Optimum}}\end{sideways} & 
\begin{minipage}{\widthCol}%
\centering%
\includegraphics[scale=0.3, trim=5cm 3cm 0cm 3cm,clip]{figuresMatlab/refinedPoses-gtsam-sphere_bignoise_vertex3-chordal} 
\end{minipage}
& 
\begin{minipage}{\widthCol}%
\centering%
\includegraphics[scale=0.3, trim=3cm 2cm 0cm 3cm,clip]{figuresMatlab/refinedPoses-gtsam-torus3D-chordal}  
\end{minipage}
\vspace{-0.1cm}
\\
%%%%%%% SECOND ROW
\begin{sideways}{$\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!${Local Minimum}}\end{sideways} &
\begin{minipage}{\widthCol}%
\centering%
\includegraphics[scale=0.26, trim=5cm 3cm 0cm 2cm,clip]{figuresMatlab/refinedPoses-odometry-sphere_bignoise_vertex3-X} 
\end{minipage}
& 
\begin{minipage}{\widthCol}%
\centering%
\includegraphics[scale=0.25, trim=3cm 1.6cm 0cm 2cm,clip]{figuresMatlab/refinedPoses-odometry-torus3D-X}
\end{minipage}
\vspace{0.1cm}
\end{tabular}%
\caption{\label{fig:maps} 
This paper exploits Lagrangian duality to evaluate the 
quality of a SLAM solution. For instance, our verification techniques
are able to certify the optimality of the solutions in the first row of the figure, 
while they reject as suboptimal the estimates shown in the bottom row.
% Examples of global and local minima in 3D pose graph optimization.
% \sphereHard and \torus datasets~\cite{Carlone15icra-init3D} 
% and in many, in figure, \grid, \cubicle, \rim.
}
\vspace{-0.3cm} 
\end{minipage}%
\end{figure}


==> maps_blueRed_all.tex <==
%!TEX root = main.tex

\definecolor{dgreen}{rgb}{0,0.5,0}

% \newcommand{\textwidth}{9cm}
\newcommand{\widthCol}{3cm}
\newcommand{\GN}{{\tt GN}\xspace}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \subsection{Simulated Datasets}
\vspace{0.5cm}

\begin{figure}[h]
\vspace{-0.5cm}
\begin{minipage}{8.5cm}%\vspace{-3mm}
% \hspace{4mm}
\begin{tabular}{ccc}%
& \color{blue}{\GN from initialization} & \hspace{0.5cm}  \color{red}{\GN from odometry}
\vspace{-0.1cm}
\\
%%%%%%% ROW
\begin{sideways}{$\!\!\!\!${\sphere}}\end{sideways} & 
\begin{minipage}{\widthCol}%
\centering%
\includegraphics[scale=0.3, trim=5cm 1cm 0cm 2cm,clip]{figuresMatlab/10iter/eps/refinedPoses-gtsam-sphere2500vertigo-chordal} 
\end{minipage}
& 
\begin{minipage}{\widthCol}%
\centering%
\includegraphics[scale=0.3, trim=4cm 1cm 1cm 2cm,clip]{figuresMatlab/10iter/eps/refinedPoses-odometry-sphere2500vertigo-X}  
\end{minipage}
\vspace{-0.6cm}
\\
%%%%%%% ROW
\begin{sideways}{$\!\!\!\!\!\!\!\!\!\!\!${\sphereHard}}\end{sideways} & 
\begin{minipage}{\widthCol}%
\centering%
\includegraphics[scale=0.32, trim=5cm 1cm 0cm 1cm,clip]{figuresMatlab/refinedPoses-gtsam-sphere_bignoise_vertex3-chordal} 
\end{minipage}
& 
\begin{minipage}{\widthCol}%
\centering%
\includegraphics[scale=0.25, trim=4cm 0cm 0cm 1cm,clip]{figuresMatlab/refinedPoses-odometry-sphere_bignoise_vertex3-X}  
\end{minipage}
\vspace{-0.6cm}
\\
%%%%%%% ROW
\begin{sideways}{$\!\!\!\!\!\!\!\!\!\!\!${\torus}}\end{sideways} & 
\begin{minipage}{\widthCol}%
\centering%
\includegraphics[scale=0.27, trim=3cm 2cm 0cm 1cm,clip]{figuresMatlab/refinedPoses-gtsam-torus3D-chordal}  
\end{minipage}
& 
\begin{minipage}{\widthCol}%
\centering%
\includegraphics[scale=0.32, trim=4cm 2cm 2cm 1cm,clip]{figuresMatlab/refinedPoses-odometry-torus3D-X}
\end{minipage}
\vspace{-0.6cm}
\end{tabular}%
\vspace{-0.3cm} 
\end{minipage}%
\end{figure}

\pagebreak

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\begin{figure}[h!]
%\vspace{-0.5cm}
%\begin{minipage}{8.5cm}%\vspace{-3mm}
%% \hspace{4mm}
%\begin{tabular}{ccc}%
%& \color{blue}{\GN from initialization} & \hspace{0.5cm}  \color{red}{\GN from odometry}
%\\
%%%%%%%% ROW
%\begin{sideways}{{\grid}}\end{sideways} & 
%\begin{minipage}{\widthCol}%
%\vspace{-0.5cm}
%\centering%
%\includegraphics[scale=0.27, trim=5cm 1cm 0cm 2cm,clip]{figuresMatlab/10iter/eps/refinedPoses-gtsam-grid3D-chordal} 
%\end{minipage}
%& 
%\begin{minipage}{\widthCol}%
%\centering%
%\includegraphics[scale=0.45, trim=6cm 1cm 0cm 2cm,clip]{figuresMatlab/10iter/eps/refinedPoses-odometry-grid3D-X}  
%\end{minipage}
%\end{tabular}%
%\end{minipage}%
%\end{figure}
%
%\vspace{1cm}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \subsection{Real Datasets}


\begin{figure}[h!]
\begin{minipage}{8.5cm}%\vspace{-3mm}
% \hspace{4mm}
\begin{tabular}{ccc}%
& \color{blue}{\GN from initialization} & \hspace{0.5cm}  \color{red}{\GN from odometry}
\vspace{-0.1cm}
\\
%%%%%%% ROW
\begin{sideways}{{\grid}}\end{sideways} & 
\begin{minipage}{\widthCol}%
\vspace{-0.5cm}
\centering%
\includegraphics[scale=0.27, trim=5cm 1cm 0cm 2cm,clip]{figuresMatlab/10iter/eps/refinedPoses-gtsam-grid3D-chordal} 
\end{minipage}
& 
\begin{minipage}{\widthCol}%
\centering%
\includegraphics[scale=0.42, trim=5cm 0cm 0cm 2cm,clip]{figuresMatlab/10iter/eps/refinedPoses-odometry-grid3D-X-manual}  
\end{minipage}
\vspace{-1.5cm}
\\
%%%%%%% ROW
\begin{sideways}{$\!\!\!\!\!\!\!\!\!\!\!${\garage}}\end{sideways} & 
\begin{minipage}{\widthCol}%
\centering%
\includegraphics[scale=0.27, trim=6cm 3cm 0cm 2cm,clip]{figuresMatlab/10iter/eps/refinedPoses-gtsam-parking-garage-chordal} 
\end{minipage}
& 
\begin{minipage}{\widthCol}%
\centering%
\includegraphics[scale=0.27, trim=5cm 2cm 0cm 2cm,clip]{figuresMatlab/10iter/eps/refinedPoses-odometry-parking-garage-X}  
\end{minipage}
\vspace{-0.6cm}
\\
\\
%%%%%%% ROW
\begin{sideways}{$\!\!\!\!\!\!\!\!\!\!\!${\cubicle}}\end{sideways} & 
\begin{minipage}{\widthCol}%
\centering%
\includegraphics[scale=0.27, trim=4.2cm 3cm 0cm 3cm,clip]{figuresMatlab/10iter/eps/refinedPoses-gtsam-cubicle-chordal} 
\end{minipage}
& 
\begin{minipage}{\widthCol}%
\centering%
\includegraphics[scale=0.3, trim=4cm 2cm 0cm 3cm,clip]{figuresMatlab/10iter/eps/refinedPoses-odometry-cubicle-X}  
\end{minipage}
\vspace{-0.6cm}
\\
\\
%%%%%%% ROW
\begin{sideways}{$\!${\rim}}\end{sideways} &
\begin{minipage}{\widthCol}%
\centering%
\includegraphics[scale=0.24, trim=3cm 2cm 0cm 2cm,clip]{figuresMatlab/10iter/eps/refinedPoses-gtsam-rim-chordal} 
\end{minipage}
& 
\begin{minipage}{\widthCol}%
\centering%
\includegraphics[scale=0.32, trim=4cm 2cm 2cm 3cm,clip]{figuresMatlab/10iter/eps/refinedPoses-odometry-rim-X}
\end{minipage}
\vspace{-0.3cm}
\end{tabular}%
\end{minipage}%
\caption{Blue: Estimated trajectory obtained by refining the \emph{chordal} initialization of~\cite{Carlone15icra-init3D} 
 with 10 Gauss-Newton iterations. Red: Estimated trajectory obtained by refining the odometric guess 
 with 10 Gauss-Newton iterations.}
\end{figure}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \subsection{The \garage dataset}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\pagebreak

\begin{figure}[h!]
\begin{minipage}{8.5cm}%\vspace{-3mm}
% \hspace{4mm}
\begin{tabular}{cc}%
\begin{sideways}{\hspace{-5cm}{\garage: zoomed-in view and comparison}}\end{sideways} & 
%%%%%%% ROW
\begin{minipage}{8.5cm}%
\vspace{0.5cm}
\centering%
\includegraphics[scale=0.4, trim=5cm 1cm 0cm 2cm,clip]{figuresMatlab/garage1} 
\end{minipage}
\\
& \begin{minipage}{8.5cm}%
\hspace{-1cm}
\centering%
\includegraphics[scale=0.25, trim=3cm 1cm 1cm 0cm,clip]{figuresMatlab/garage2}  
\end{minipage}
\end{tabular}%
\end{minipage}%
\caption{\garage dataset: while the estimates obtained from \GN with initialization (blue) and 
\GN from odometry (red) attain a very similar cost ($6.2994\e^{-1}$ versus $6.2997\e^{-1}$), 
the corresponding trajectories are still different, which indicates that \GN from odometry 
did not completely converge after 10 iterations.}
\end{figure}

\vspace{1cm}

==> rotationDerivation.tex <==
%!TEX root = main.tex

\section{3D Rotation Graph Optimization}

Let us consider the case in which a rotation $\MR_i \in\SOthree$ is associated 
to each edge in the graph and we want to estimate these rotations from relative 
rotation measurements $\MRij$, $(i,j)\in\calE$.

Under this setup, that we call Rotation Graph Optimization, we estimate rotations 
by minimizing the following cost:
\bea
\label{eq:OGO}
f_r^\star = 
\min_{\{ \MR_i \in \SOthree \}}
\sumalledges \normsq{ \MR_i \MRij - \MR_j }{\frob} 
\eea
%
which can be readily seen to coincide with the second summand in~\eqref{eq:PGO}.


\subsection{Reformulating~\eqref{eq:OGO} as a quadratic problem with quadratic equality constraints}

The first step is to make explicit the constraint that $\MR_i$ is a rotation matrix:
%
\bea
\label{eq:OGO2}
f_r^\star &=& 
\min_{\{ \MR_i \}}
\sumalledges \normsq{ \MR_i \MRij - \MR_j }{\frob}  \nonumber \\
\subject && 
\left.
\begin{array}{c}
\MR_i\tran \MR_i = \eye_3 \\
\det(\MR_i) = 1
\end{array}
\right\}
 \quad i=1,\ldots,n 
\eea
%
The determinant might be more difficult to tackle so we start with a relaxed 
version of the problem, which neglects this constraint (\LC{later we have to 
work out the implication of this}). Neglecting the determinant constraint we get:
%
\bea
\label{eq:primalOGO}
\tilde f_r^\star &=& 
\min_{\{ \MR_i \}}
\sumalledges \normsq{ \MR_i \MRij - \MR_j }{\frob}  \nonumber \\
\subject && 
\MR_i\tran \MR_i = \eye_3,
 \quad i=1,\ldots,n 
\eea
%
If we call $\vr_i^k$ the $k$-th row of $\MR_i$ (written as a column vector), 
and we define $\vr_i =[(\vr_i^1)\tran \; (\vr_i^2)\tran \; (\vr_i^3)\tran]\tran \in \Real{9}$ 
(vectorization of $\MR_i$), the following equality holds:
%
\bea
\label{eq:vectorRij}
\normsq{ \MR_i \MRij - \MR_j }{\frob} = \sum_{k=1}^3 \normsq{\MRij\tran \vr_i^k - \vr_j^k}{}
= \normsq{\bigMRij \vr_i - \vr_j}{}
\eea
%
where $\bigMRij \in \Real{9 \times 9}$ is a block diagonal matrix.
%
Using~\eqref{eq:vectorRij}, problem~\eqref{eq:primalOGO} becomes:
%
\bea
\label{eq:primalOGOvect}
\tilde f_r^\star &=&
\min_{\{ \vr_i \}}
\sumalledges \normsq{\bigMRij \vr_i - \vr_j}{}  \\
\subject & &
\left.
\begin{array}{ll}
\vr_i\tran \ME_{jj} \vr_i = 1, & j=1,2,3 \\
\vr_i\tran \ME_{jk} \vr_i = 0, & k \neq j \\
\end{array}
\right\}
 \; i=1,\ldots,n \nonumber
\eea
%
where $\MR_{jk} \in \Real{9\times 9}$ are matrices that are all zeros except a $3\times 3$ 
identity block.

If we stack all $\vr_i$ in a vector $\vr \in \Real{9\nrNodes}$, we can write~\eqref{eq:primalOGOvect}: 
%
\bea
\label{eq:primalOGOr0}
\tilde f_r^\star &=&
\min_{\vr}
\normsq{ \MA \vr }{} \\
\subject & &
\left.
\begin{array}{ll}
\vr\tran \ME_{ijj} \vr = 1, & j=1,2,3 \\
\vr\tran \ME_{ijk} \vr = 0, & k \neq j \\
\end{array}
\right\}
 \; i=1,\ldots,n \nonumber
\eea
% 
where now $\ME_{ijk}$ are larger sparse matrices.

Defining a matrix $\MQ \doteq \MA\tran \MA$, the previous problem becomes 
%
\bea
\label{eq:primalOGOr}
\tilde f_r^\star &=&
\min_{\vr}
\vr\tran \MQ \vr  \\
\subject & &
\left.
\begin{array}{ll}
\vr\tran \ME_{ijj} \vr = 1, & j=1,2,3 \\
\vr\tran \ME_{ijk} \vr = 0, & k \neq j \\
\end{array}
\right\}
 \; i=1,\ldots,n \nonumber
\eea
% 

\section{The dual of problem~\eqref{eq:primalOGOr}}

The Lagrangian of the primal problem~\eqref{eq:primalOGOr} is:
\bea
\calL(\vr,\lam) = \vr\tran \MQ \vr + 
\sum_{i=1}^n \bigg[
\sum_{j=1,2,3} \lamPara_{ij} (1 - \vr\tran \ME_{ijj} \vr)  + \\ 
\sum_{j,k=1,2,3, \; k>j} \lamPerp_{ijk} (-\vr\tran \ME_{ijk} \vr)
\bigg]
\eea
%
where $\lamPara_{ij}$ are the Lagrange multipliers associated 
with the unit norm constraints in~\eqref{eq:primalOGOr}, while 
$\lamPerp_{ijk}$ are the multipliers associated with the perpendicularity constraints in~\eqref{eq:primalOGOr}.
(\LC{notation is a bit heavy here, but we can simplify later..}).
We denote with $\vlam$ the vector stacking all Lagrange multipliers.

Rearranging the terms we get:
%
\bea
\label{eq:lagrangian}
\calL(\vr,\lam) = \vr\tran \hat \MQ(\vlam) \vr 
+ \sum_{i=1}^n 
\sum_{j=1,2,3} \lamPara_{ij}
\eea
%
where:
%
\bea
\label{eq:defQlambda}
\hat{\MQ}(\vlam) = \MQ - \sum_{i=1}^n \bigg[
\sum_{j=1,2,3} \lamPara_{ij} \ME_{ijj}  +  
\sum_{j,k=1,2,3, \; k>j} \lamPerp_{ijk} \ME_{ijk}
\bigg]
\eea
%

The \emph{dual function} is then defined as the infimum of the Lagrangian with respect to $\vr$:
%
\bea
\label{eq:dualFunction}
d(\vlam) = \inf_{\vr} \vr\tran \hat \MQ(\vlam) \vr 
+ \sum_{i=1}^n 
\sum_{j=1,2,3} \lamPara_{ij}
\eea
%

Which leads to the definition of our \emph{dual problem}:
%
\bea
\label{eq:dualProblem}
d^\star = \max_{\vlam} \; \inf_{\vr} d(\vlam) = 
\max_{\vlam} \; \inf_{\vr} \vr\tran \hat \MQ(\vlam) \vr 
+ \sum_{i=1}^n 
\sum_{j=1,2,3} \lamPara_{ij}
\eea
%

The optimal dual cost $d^\star$ drifts to minus infinity if $\hat \MQ(\vlam)$ 
is negative definite. Since we are looking for the maximum over $\vlam$  
 we can safely restrict our search to the vectors $\vlam$ that preserve semi-definiteness of $\hat \MQ(\vlam)$.
 Accordingly,~\eqref{eq:dualProblem} becomes:
%
\bea
\label{eq:dualProblemSDP}
d^\star &=& \max_{\vlam} \;  \sum_{i=1}^n 
\sum_{j=1,2,3} \lamPara_{ij} \nonumber \\
\subject && \MQ(\vlam) \succeq 0
\eea
%
The dual problem~\eqref{eq:dualProblemSDP} is an SDP and can be solved via convex programming.
Also, the following inequality holds:
\beq
d^\star \leq \tilde{f}_r^\star \quad \text{(weak duality)}
\eeq 
%
hence $d^\star$ can be used as a lower bound for the 
optimal cost $\tilde{f}_r^\star$ of the primal problem~\eqref{eq:primalOGOr}.

\begin{remark}
It turns out that the bound $d^\star$ produced by the dual problem is quite loose, i.e., 
in practical problems $d^\star \ll \tilde{f}_r^\star$. This motivates the development 
in the following section.
\end{remark}


\section{Duality 2.0}

Let us restart from the primal problem given in~\eqref{eq:primalOGOr0}, that we 
restate here:
%
\bea
\label{eq:primalOGOrRepeat}
\tilde f_r^\star &=&
\min_{\vr}
\normsq{ \MA \vr }{} \\
\subject & &
\left.
\begin{array}{ll}
\vr\tran \ME_{ijj} \vr = 1, & j=1,2,3 \\
\vr\tran \ME_{ijk} \vr = 0, & k \neq j \\
\end{array}
\right\}
 \; i=1,\ldots,n \nonumber
\eea
% 
This problem has a rotational symmetry, as we can substitute 
the rotations $\MR_i$, $i=1,\ldots,\nrNodes$, with $\MS \MR_i$ ($\MS \in \SOthree$), without 
altering the cost (and satisfying the constraints). This is due to the 
fact that we cannot observe global rotation from relative rotation measurements.

In this section we prefer to remove this symmetry before applying duality theory.

\subsection{Anchoring}

We remove the rotational ambiguity by fixing the rotation at one of the nodes.
Without loss of generality we fix the rotation of the first node to the identity matrix.
This is equivalent to setting $\vr_1 = [\ve_1 \; \ve_2 \; \ve_3]$, where $\ve_i$ 
is a vector that contains 1 at the $i$-th entry, and is zero elsewhere. The process 
of fixing a node to remove the rotational ambiguity is usually referred to as \emph{anchoring}.

After anchoring, the primal~\eqref{eq:primalOGOrRepeat} becomes:
%
\bea
\label{eq:primalOGOrAnchoring}
\tilde f_r^\star &=&
\min_{\vr}
\normsq{ \MA \vr - \vb }{} \\
\subject & &
\left.
\begin{array}{ll}
\vr\tran \ME_{ijj} \vr = 1, & j=1,2,3 \\
\vr\tran \ME_{ijk} \vr = 0, & k \neq j \\
\end{array}
\right\}
 \; i=1,\ldots,n \nonumber
\eea
%
where, with slight abuse of notation, we use $\vr \in \Real{9(n-1)}$ to denote the vector of unknown rotations 
(without the node 1), and $\vb \doteq - \MA \vr_1$.

\subsection{Duality}

We can rewrite the cost in~\eqref{eq:primalOGOrAnchoring} as follows:
\bea
\normsq{ \MA \vr - \vb }{} = \vr\tran \MA\tran \MA \vr - 2 \vb\tran \MA \vr + \vb\tran \vb = \\
\left[
\ba{cc}
\vr \\
1
\ea
\right]\tran
\left[
\ba{cc}
\MA\tran \MA  & - \MA\tran \vb\\
- \vb\tran \MA & \vb\tran \vb
\ea
\right]
\left[
\ba{cc}
\vr \\
1
\ea
\right]
\eea
%
which allows to rewrite~\eqref{eq:primalOGOrAnchoring} as:
%
\bea
\label{eq:primalOGOhom0}
\tilde f_r^\star &=&
\min_{\vr}
\left[
\ba{cc}
\vr \\
1
\ea
\right]\tran
\left[
\ba{cc}
\MA\tran \MA  & - \MA\tran \vb\\
- \vb\tran \MA & \vb\tran \vb
\ea
\right]
\left[
\ba{cc}
\vr \\
1
\ea
\right]
 \\
\subject & &
\left.
\begin{array}{ll}
\vr\tran \ME_{ijj} \vr = 1, & j=1,2,3 \\
\vr\tran \ME_{ijk} \vr = 0, & k \neq j \\
\end{array}
\right\}
 \; i=1,\ldots,n \nonumber 
\eea
%

The Lagrangian of~\eqref{eq:primalOGOhom0} is:
%
\bea
\label{eq:lagrangian2}
\calL(\vr,\lam) = \left[
\ba{cc}
\vr \\
1
\ea
\right]\tran 
\MM(\lambda)
\left[
\ba{cc}
\vr \\
1
\ea
\right] 
\eea%\
%
where $\MM(\lambda) =$

\tiny
\bea
\left[
\ba{cc}
\displaystyle \MA\tran \MA -  \sum_{i=1}^n \bigg[
\sum_{j=1,2,3} \lamPara_{ij} \ME_{ijj} - 
\sum_{k \neq j} \lamPerp_{ijk} \ME_{ijk} \bigg]  & - \MA\tran \vb\\
- \vb\tran \MA & \vb\tran \vb + \sum_{i=1}^n 
\sum_{j=1,2,3} \lamPara_{ij} \ME_{ijj}
\ea
\right]
\eea

% \sum_{i=1}^n \bigg[
% \sum_{j=1,2,3} \lamPara_{ij} (1 - \vr\tran \ME_{ijj} \vr)  + \\ 
% \sum_{j,k=1,2,3, \; k>j} \lamPerp_{ijk} (-\vr\tran \ME_{ijk} \vr)
% \subsection{Homogenization}

\normalsize

The dual problem is then:
%
\bea
\label{eq:dual2}
d^\star_2 = \max_\lam \min_\vr 
\left[
\ba{cc}
\vr \\
1
\ea
\right]\tran 
\MM(\lambda)
\left[
\ba{cc}
\vr \\
1
\ea
\right] 
\eea%\
%

We can \emph{homogenize} the cost~\eqref{eq:dual2} by adding a slack variable 
$q$ and the corresponding Lagrange multiplier $\gamma$ \LC{TODO: add extra 
explanation here, also, cite [Frederikson12accv] which does quite the same with quaternions}:
%
\bea
\label{eq:dual3}
d^\star_2 =&  \max_\lam \min_\vr &
\left[
\ba{cc}
\vr \\
q
\ea
\right]\tran 
\breve\MM(\lambda,\gamma)
\left[
\ba{cc}
\vr \\
q
\ea
\right] + \gamma
\eea
%
where $\breve \MM(\lambda,\gamma) =$

\tiny
\bea
\left[
\ba{cc}
\displaystyle \MA\tran \MA -  \sum_{i=1}^n \bigg[
\sum_{j=1,2,3} \lamPara_{ij} \ME_{ijj} - 
\sum_{k \neq j} \lamPerp_{ijk} \ME_{ijk} \bigg]  & - \MA\tran \vb\\
- \vb\tran \MA & \vb\tran \vb + \sum_{i=1}^n 
\sum_{j=1,2,3} \lamPara_{ij} \ME_{ijj} -\gamma
\ea
\right]
\eea

\normalsize

This finally leads to our dual problem:
%
\bea
\label{eq:dual3}
d^\star_2 =&  \max_\lam & \gamma \\
& \subject & \MM(\lam,\gamma)\succeq 0
\eea
%

==> table.tex <==
%!TEX root = main.tex

\renewcommand{\e}[1]{\cdot 10^{#1}}

\newcommand{\red}[1]{{\color{red}#1}}
\newcommand{\green}[1]{{\color{green}#1}}
\newcommand{\good}[1]{{\color{blue}#1}}%\bm{}
\newcommand{\no}{$-$}
\newcommand{\myfont}[1]{{\small #1}}
\newcommand{\brac}{\bigg\}}
\newcommand{\fang}{f_{\mbox{ang}}}
\newcommand{\fchord}{f_{\mbox{chord}}}

\newcommand{\extraCol}[1]{#1}

\begin{center}
\begin{table*}[t]
\renewcommand*\arraystretch{1.1}
\begin{centering}
{\scriptsize 
\begin{tabular}{|  c | c || c | c | c | c  c | c | c | c |}
\hline
&  & $f_{\text{GN}}$ & $d(\vlamHat)$ & $r$ & \multicolumn{2}{c|}{$\mu^{-}$}  & Time & Certificate \\
\hline
\hline
%==================================================================== 
\sphere & Init. & $5.7595\e{2}$  & $5.75\e{2}$ & $8.92\e{-6}$ & $0\e{0}$ & ($-1.81\e{-4}$) & $609.14$ & \green{\checkmark} \\ 
$\substack{ n=2500 \\ m=4949}$ & Odom. & \red{$5.8019\e{2}$}  & \red{$4.38\e{2}$} & $1.58\e{-4}$ & $0\e{0}$ & ($-1.45\e{-4}$) & $597.31$ & \red{x} \\ 
\hline 
%==================================================================== 
\sphereHard & Init. & $1.2485\e{6}$  & $1.25\e{6}$ & $1.47\e{-3}$ & $-9.64\e{-3}$ & ($-9.64\e{-3}$) & $332.62$ & \green{\checkmark} \\ 
$\substack{ n=2200 \\ m=8647}$ & Odom. & \red{$3.0413\e{6}$}  & $3.04\e{6}$ & \red{$7.96\e{-1}$} & \red{$-1.01\e{2}$} & (\red{$-5.82\e{3}$}) & $2.51$ & \red{x} \\ 
\hline 
%==================================================================== 
\torus & Init. & $1.2114\e{4}$  & $1.21\e{4}$ & $8.19\e{-6}$ & $-7.85\e{-2}$ & ($-7.85\e{-2}$) & $39.52$ & \green{\checkmark} \\ 
$\substack{ n=5000 \\ m=9048}$ & Odom. & \red{$2.7666\e{4}$}  & $2.76\e{4}$ & $1.12\e{-3}$ & \red{$-1.04\e{2}$} & (\red{$-1.37\e{2}$}) & $3.73$ & \red{x} \\ 
\hline 
%==================================================================== 
\grid & Init. & $4.216\e{4}$  & $4.22\e{4}$ & $6.78\e{-6}$ & $-1.24\e{-2}$ & ($0\e{0}$) & $1646.31$ & \green{\checkmark} \\ 
$\substack{ n=8000 \\ m=22236}$ & Odom. & \red{$2.7465\e{5}$}  & $2.74\e{5}$ & $2.14\e{-2}$ & \red{$-9.98\e{1}$} & ($0\e{0}$) & $68.17$ & \red{x} \\ 
\hline 
%==================================================================== 
\garage & Init. & $6.2994\e{-1}$  & $6.11\e{-1}$ & $1.63\e{-7}$ & $-6.78\e{-2}$ & ($-6.78\e{-2}$) & $12.34$ & \green{\checkmark} \\ 
$\substack{ n=1661 \\ m=6275}$ & Odom. & $6.2997\e{-1}$  & \red{$3.53\e{-1}$} & $6.23\e{-7}$ & $-6.75\e{-2}$ & ($-6.75\e{-2}$) & $11.20$ & \red{x} \\ 
\hline 
%==================================================================== 
\cubicle & Init. & $6.2481\e{2}$  & $6.25\e{2}$ & $1.93\e{-7}$ & $-4.76\e{-1}$ & ($0\e{0}$) & $16.85$ & \green{\checkmark} \\ 
$\substack{ n=5750 \\ m=16869}$ & Odom. & $6.2484\e{2}$  & $6.16\e{2}$ & $2.35\e{-5}$ & $-4.75\e{-1}$ & ($0\e{0}$) & $15.51$ & \green{\checkmark} \\ 
\hline 
%==================================================================== 
\rim & Init. & $1.235\e{4}$  & $1.23\e{4}$ & $1.4\e{-5}$ & \red{$-9.77\e{1}$} & ($0\e{0}$) & $7.71$ & \red{x} \\ 
$\substack{ n=10195 \\ m=29743}$ & Odom. & \red{$1.6985\e{4}$}  & \red{$-2.8\e{4}$} & $8.5\e{-3}$ & \red{$-9.38\e{1}$} & ($0\e{0}$) & $7.06$ & \red{x} \\ 
\hline 

\end{tabular}
}
\vspace{0.1cm}
\caption{Cost attained in~\eqref{eq:general}, CPU time, and number of Gauss-Newton iterations for different benchmarking problems, comparing the odometric cost, the cost attained by  \gtwoo and \gtsam, and 
\label{tab:real}}
\end{centering}
\vspace{-0.8cm}
\end{table*}
\end{center}


==> table2.tex <==
%!TEX root = main.tex

\renewcommand{\e}[1]{\cdot 10^{#1}}

\newcommand{\red}[1]{{\color{red}#1}}
\newcommand{\green}[1]{{\color{green}#1}}
\newcommand{\good}[1]{{\color{blue}#1}}%\bm{}
\newcommand{\no}{$-$}
\newcommand{\myfont}[1]{{\small #1}}
\newcommand{\brac}{\bigg\}}
\newcommand{\fang}{f_{\mbox{ang}}}
\newcommand{\fchord}{f_{\mbox{chord}}}

\newcommand{\showMuFull}[1]{} %{#1}

\newcommand{\extraCol}[1]{#1}

\begin{center}
\begin{table*}[t]
\renewcommand*\arraystretch{1.1}
\begin{centering}
{\scriptsize 
\begin{tabular}{|  c | c || c | c | c  | c | c | c |}
\hline
&  & $\fML(\hat\vxx)$ & $d(\vlamHat)$ & $\mu$ \showMuFull{\multicolumn{2}{c|}{$\mu^{-}$}}  & Time & Certificate \\
\hline
\hline
%==================================================================== 
\sphere & Init. & $5.7595\e{2}$  & $5.75\e{2}$ & $0$ \showMuFull{& ($-1.81\e{-4}$)} & $609.14$ & \green{\checkmark} \\ 
$\substack{ n=2500 \\ m=4949}$ & Odom. & \red{$5.8019\e{2}$}  & \red{$4.38\e{2}$} & $0$ \showMuFull{& ($-1.45\e{-4}$)} & $597.31$ & \red{x} \\ 
\hline 
%==================================================================== 
\sphereHard & Init. & $1.2485\e{6}$  & $1.25\e{6}$ & $-9.64\e{-3}$ \showMuFull{& ($-9.64\e{-3}$)} & $332.62$ & \green{\checkmark} \\ 
$\substack{ n=2200 \\ m=8647}$ & Odom. & \red{$3.0413\e{6}$}  & $3.04\e{6}$ & \red{$-1.01\e{2}$} \showMuFull{& (\red{$-5.82\e{3}$})} & $2.51$ & \red{x} \\ 
\hline 
%==================================================================== 
\torus & Init. & $1.2114\e{4}$  & $1.21\e{4}$ & $-7.85\e{-2}$ \showMuFull{& ($-7.85\e{-2}$)} & $39.52$ & \green{\checkmark} \\ 
$\substack{ n=5000 \\ m=9048}$ & Odom. & \red{$2.7666\e{4}$}  & $2.76\e{4}$ & \red{$-1.04\e{2}$} \showMuFull{& (\red{$-1.37\e{2}$})} & $3.73$ & \red{x} \\ 
\hline 
%==================================================================== 
\grid & Init. & $4.216\e{4}$  & $4.22\e{4}$ & $-1.24\e{-2}$ \showMuFull{& (--)} & $1646.31$ & \green{\checkmark} \\ 
$\substack{ n=8000 \\ m=22236}$ & Odom. & \red{$2.7465\e{5}$}  & $2.74\e{5}$ & \red{$-9.98\e{1}$} \showMuFull{& (--)} & $68.17$ & \red{x} \\ 
\hline 
%==================================================================== 
\garage & Init. & $6.2994\e{-1}$  & $6.11\e{-1}$ & $-6.78\e{-2}$ \showMuFull{& ($-6.78\e{-2}$)} & $12.34$ & \green{\checkmark} \\ 
$\substack{ n=1661 \\ m=6275}$ & Odom. & $6.2997\e{-1}$  & \red{$3.53\e{-1}$} & $-6.75\e{-2}$ \showMuFull{& ($-6.75\e{-2}$)} & $11.20$ & \red{x} \\ 
\hline 
%==================================================================== 
\cubicle & Init. & $6.2481\e{2}$  & $6.25\e{2}$ & $-4.76\e{-1}$ \showMuFull{& (--)} & $16.85$ & \green{\checkmark} \\ 
$\substack{ n=5750 \\ m=16869}$ & Odom. & $6.2484\e{2}$  & $6.16\e{2}$ & $-4.75\e{-1}$ \showMuFull{& (--)} & $15.51$ & \green{\checkmark} \\ 
\hline 
%==================================================================== 
\rim & Init. & $1.235\e{4}$  & $1.23\e{4}$ & \red{$-9.77\e{1}$} \showMuFull{& (--)} & $7.71$ & \red{x} \\ 
$\substack{ n=10195 \\ m=29743}$ & Odom. & \red{$1.6985\e{4}$}  & \red{$-2.8\e{4}$} & \red{$-9.38\e{1}$} \showMuFull{& (--)} & $7.06$ & \red{x} \\ 
\hline 

\end{tabular}
}
\vspace{0.1cm}
\caption{Cost attained in~\eqref{eq:general}, CPU time, and number of Gauss-Newton iterations for different benchmarking problems, comparing the odometric cost, the cost attained by  \gtwoo and \gtsam, and 
\label{tab:real}}
\end{centering}
\vspace{-0.8cm}
\end{table*}
\end{center}


==> tableInit.tex <==
%!TEX root = main.tex

\renewcommand{\e}[1]{\cdot 10^{#1}}

\newcommand{\red}[1]{{\color{red}#1}}
\newcommand{\good}[1]{{\color{blue}#1}}%\bm{}
\newcommand{\no}{$-$}
\newcommand{\myfont}[1]{{\small #1}}
\newcommand{\brac}{\bigg\}}


\newcommand{\extraCol}[1]{#1}

\begin{center}
\begin{table*}[t]
\renewcommand*\arraystretch{1.1}
\begin{centering}
{\scriptsize 
\begin{tabular}{|  c | c || c | cc | c | cc | ccc |}
\hline
& &  \myfont{odometry} & \myfont{\gtwoo} & \myfont{\gtwooST} & \myfont{\gtsam}  & \multicolumn{2}{c|}{\myfont{a}}  &  \multicolumn{3}{c|}{\myfont{b}}  \\
\hline
\hline
%==================================================================== 
\myfont{\sphere} & Iter. & \no & $5$ & $5$ & $7$ & $1$ & $4$ & $1$ & $5$ & \multirow{3}{*}{$\!\!\!\! \brac 1435$}\\ 
$n=2500$ & Cost & $\! 1.29\e{6} \!$ & $\! 4.39\e{3} \!$ & $\! 7.91\e{2} \!$ & $\! \good{6.76\e{2}} \!$ & $\! 9.63\e{2} \!$ & $\! \good{6.76\e{2}} \!$ & $\! 1.24\e{4} \!$ & $\! \good{6.76\e{2}} \!$ & \\ 
$m=4949$ & Time &  \no & $1.19$ & $1.23$  & $0.96$ & $0.52$ & $0.85$ & $6.40$ & $6.89$ &\\ 
\hline 
%==================================================================== 
\myfont{\sphereHard} & Iter. & \no & $5$ & $5$ & $1$ & $1$ & $4$ & $1$ & $1$ & \multirow{3}{*}{$\!\!\!\! \brac 8155$}\\ 
$n=2200$ & Cost & $\! 1.34\e{8} \!$ & $\! \red{5.32\e{10}} \!$ & $\! 5.43\e{6} \!$ & $\! \red{5.71\e{10}} \!$ & $\! 1.51\e{6} \!$ & $\! \good{1.49\e{6}} \!$ & $\! \red{1.9\e{6}} \!$ & $\! \red{1.9\e{6}} \!$ & \\ 
$m=8647$ & Time &  \no & $2.46$ & $2.48$  & $0.46$ & $0.79$ & $1.28$ & $50.26$ & $50.87$ &\\ 
\hline 
%==================================================================== 
\myfont{\torus} & Iter. & \no & $5$ & $5$ & $2$ & $1$ & $4$ & $1$ & $12$ & \multirow{3}{*}{$\!\!\!\! \brac 1231$}\\ 
$n=5000$ & Cost & $\! 1.99\e{6} \!$ & $\! \red{6.04\e{8}} \!$ & $\! 1.27\e{4} \!$ & $\! 4.71\e{10} \!$ & $\! 1.24\e{4} \!$ & $\! \good{1.21\e{4}} \!$ & $\! \red{5.85\e{4}} \!$ & $\! \red{2.81\e{4}} \!$ & \\ 
$m=9048$ & Time &  \no & $3.90$ & $3.90$  & $0.83$ & $1.18$ & $1.97$ & $11.35$ & $14.45$ &\\ 
\hline 
%==================================================================== 
\myfont{\grid} & Iter. & \no & $5$ & $5$ & $2$ & $1$ & $4$ & $1$ & $4$ & \multirow{3}{*}{$\!\!\!\! \brac 1045$}\\ 
$n=8000$ & Cost & $\! 7.32\e{7} \!$ & $\! \red{5.39\e{7}} \!$ & $\! 4.6\e{4} \!$ & $\! 6.58\e{11} \!$ & $\! 4.51\e{4} \!$ & $\! \good{4.22\e{4}} \!$ & $\! 4.61\e{4} \!$ & $\! \good{4.22\e{4}} \!$ & \\ 
$m=22236$ & Time &  \no & $188.08$ & $187.32$  & $15.80$ & $31.33$ & $53.78$ & $31.60$ & $54.80$ &\\ 
\hline 
%==================================================================== 
\myfont{\garage} & Iter. & \no & $5$ & $5$ & $4$ & $1$ & $4$ & $1$ & $4$ & \multirow{3}{*}{$\!\!\!\! \brac 234$}\\ 
$n=1661$ & Cost & $\! 8.36\e{3} \!$ & $\! 6.43\e{-1} \!$ & $\! 6.43\e{-1} \!$ & $\! 6.35\e{-1} \!$ & $\! 1.51\e{0} \!$ & $\! \good{6.35\e{-1}} \!$ & $\! 1.12\e{1} \!$ & $\! \good{6.35\e{-1}} \!$ & \\ 
$m=6275$ & Time &  \no & $0.32$ & $0.33$  & $0.43$ & $0.32$ & $0.48$ & $1.23$ & $1.42$ &\\ 
\hline 
%==================================================================== 
\myfont{\cubicle} & Iter. & \no & $5$ & $5$ & $1$ & $1$ & $4$ & $1$ & $5$ & \multirow{3}{*}{$\!\!\!\! \brac 10000$}\\ 
$n=5750$ & Cost & $\! 4.99\e{6} \!$ & $\! \red{5.16\e{21}} \!$ & $\! \red{8.65\e{23}} \!$ & $\! 5.91\e{7} \!$ & $\! 8.02\e{4} \!$ & $\! \good{1.62\e{3}} \!$ & $\! 1.7\e{6} \!$ & $\! \good{1.62\e{3}} \!$ & \\ 
$m=16869$ & Time &  \no & $4.25$ & $4.28$  & $0.78$ & $1.34$ & $2.50$ & $145.46$ & $145.60$ &\\ 
\hline 
%==================================================================== 
\myfont{\rim} & Iter. & \no & $5$ & $5$ & $1$ & $1$ & $5$ & $1$ & $1$ & \multirow{3}{*}{$\!\!\!\! \brac 10000$}\\ 
$n=10195$ & Cost & $\! 4.5\e{7} \!$ & $\! \red{9.37\e{21}} \!$ & $\! \red{1.82\e{25}} \!$ & $\! 6.78\e{8} \!$ & $\! 1.31\e{6} \!$ & $\! \good{6.63\e{4}} \!$ & $\! \red{4.86\e{7}} \!$ & $\! \red{4.86\e{7}} \!$ & \\ 
$m=29743$ & Time &  \no & $7.52$ & $7.83$  & $1.42$ & $2.59$ & $5.06$ & $293.18$ & $289.08$ &\\ 
\hline  
\end{tabular}
}
\vspace{0.1cm}
\caption{Cost attained in~\eqref{eq:general}, CPU time, and number of Gauss-Newton iterations for different benchmarking problems, comparing the odometric cost, the cost attained by  \gtwoo and \gtsam, and 
\label{tab:real}}
\label{table}
\end{centering}
\vspace{-0.8cm}
\end{table*}
\end{center}

